Rate of convergence of attractors for semilinear singularly perturbed problems: scalar parabolic equations with localized large diffusion

In this paper we study the asymptotic nonlinear dynamics of scalar semilinear parabolic problems reaction-diffusion type when the diffusion coefficient becomes large in a subregion which is interior to the domain. We obtain, under suitable assumptions, that the family of attractors behaves continuously and we exhibit the rate of convergence. An accurate description of localized large diffusion is necessary.

==> References <==
% This file was created with JabRef 2.10b2.
% Encoding: UTF-8


@Book{A.N.Carvalho2010,
  Title                    = {Attractors for infinite-dimensional non-autonomous dynamical systems},
  Author                   = {A. N. Carvalho, J.A. Langa, J.C. Robinson,},
  Editor                   = {Springer},
  Year                     = {2010},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{E.R.Aragao-Costa2011,
  Title                    = {Stability of gradient semigroups under perturbations},
  Author                   = {E.R. Aragão-Costa, t. Caraballo, A. N. Carvalho, J.A.Langa},
  Journal                  = {Nonlinearity},
  Year                     = {2011},
  Volume                   = {24},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Book{Henry1980,
  Title                    = {Geometric theory of semilinear parabolic equations},
  Author                   = {Dan Henry},
  Editor                   = {Springer-Verlag},
  Publisher                = {Lecture Notes in Mathe\-matics},
  Year                     = {1980},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}



==> References.tex <==
% This file was created with JabRef 2.10b2.
% Encoding: UTF-8


@Book{A.N.Carvalho2010a,
  Title                    = {Attractors for infinite-dimensional non-autonomous dynamical systems},
  Author                   = {A. N. Carvalho, J.A. Langa, J.C. Robinson,},
  Editor                   = {Springer},
  Year                     = {2010},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{flank,
  Title                    = {Rate of convergence of Attractors for some sinsingular perturbed parabolic problems},
  Author                   = {J. M. Arrieta and F.D.M. Bezerra and A. N. Carvalho},
  Journal                  = {Top. Methdos Nonlinear Anal},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000,
  Title                    = {Attractors for parabolic pro\-blems with nonlinear boundary bondition. Uniform bounds},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Commun. in partial differential equations},
  Year                     = {2000},
  Pages                    = {1-37},
  Volume                   = {25},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000a,
  Title                    = {Upper semicontinuity for attractors of parabolic problems with localized large diffusion and nonlinear boundary conditions},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {2000},
  Pages                    = {33-59},
  Volume                   = {168},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta1999,
  Title                    = {Parabolic problems with nonlinear boundary conditions and critical nonlinearities},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {1999},
  Pages                    = {376-406},
  Volume                   = {156},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carbone2006,
  Title                    = {Continuity of the attractors in a singular problem arising in composite materials},
  Author                   = {V. L. Carbone and J. G. Ruas-Filho},
  Journal                  = {Nonlinear Anal},
  Year                     = {2006},
  Pages                    = {1285-1305},
  Volume                   = {65},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carvalho2010,
  Title                    = {Equi-exponential attraction and rate of convergence of attractors for singularly pertubed evolution equations},
  Author                   = {A.N. Carvalho and J.W. Cholewa and T.Dlotko},
  Journal                  = {Cadernos de matemática},
  Year                     = {2010},
  Pages                    = {111-151},
  Volume                   = {11},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{E.R.Aragao-Costa2011,
  Title                    = {Stability of gradient semigroups under perturbations},
  Author                   = {E.R. Aragão-Costa, T. Caraballo, A. N. Carvalho, J.A.Langa},
  Journal                  = {Nonlinearity},
  Year                     = {2011},
  Volume                   = {24},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Book{Henry1980a,
  Title                    = {Geometric theory of semilinear parabolic equations},
  Author                   = {Dan Henry},
  Editor                   = {Springer-Verlag},
  Publisher                = {Lecture Notes in Mathe\-matics},
  Year                     = {1980},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@PhdThesis{Pires2013,
  Title                    = {Taxa de atração para equações com difusão grande localizada},
  Author                   = {Leonardo Pires},
  School                   = {UfSCar},
  Year                     = {2013},
  Type                     = {Dissetação de mestrado},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Santamaria2014,
  Title                    = {Estimates on the distance of inertial manifolds},
  Author                   = {E. Santamaria and J. M. Arrieta},
  Journal                  = {Discrete and continuous dinamical systems},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {3921-3944},
  Volume                   = {34},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}


